Joint Learning of Salient Object Detection, Depth Estimation and Contour Extraction

Benefiting from color independence, illumination invariance and location discrimination attributed by the depth map, it can provide important supplemental information for extracting salient objects in complex environments. However, high-quality depth sensors are expensive and can not be widely applied. While general depth sensors produce the noisy and sparse depth information, which brings the depth-based networks with irreversible interference. In this paper, we propose a novel multi-task and multi-modal filtered transformer (MMFT) network for RGB-D salient object detection (SOD). Specifically, we unify three complementary tasks: depth estimation, salient object detection and contour estimation. The multi-task mechanism promotes the model to learn the task-aware features from the auxiliary tasks. In this way, the depth information can be completed and purified. Moreover, we introduce a multi-modal filtered transformer (MFT) module, which equips with three modality-specific filters to generate the transformer-enhanced feature for each modality. The proposed model works in a depth-free style during the testing phase. Experiments show that it not only significantly surpasses the depth-based RGB-D SOD methods on multiple datasets, but also precisely predicts a high-quality depth map and salient contour at the same time. And, the resulted depth map can help existing RGB-D SOD methods obtain significant performance gain. The source code will be publicly available at https://github.com/Xiaoqi-Zhao-DLUT/MMFT.

==> MMFT-TIP(2)/table/ablation_study_depth_estimation.tex <==
\begin{tabular}{c|cccc|ccc}
			\toprule[1.5pt]
			\multicolumn{1}{c|}{\multirow{2}*{Method}} &\multicolumn{4}{c|}{{Error}} & \multicolumn{3}{c}{{Accuracy}}\\
			
			\cmidrule(r){2-5} \cmidrule(r){6-8} 
			& RMSE $\downarrow$   & RMSE (log) $\downarrow$
			& Abs Rel $\downarrow$   & Sq ReL $\downarrow$ & P1 $\uparrow$   & P2 $\uparrow$   
			& P3 $\uparrow$   
			\\
			\midrule[1pt]
			Model 1&0.424&	0.085&	0.180&	0.120&  0.670&	0.851&	0.970  \\
			Model 2&0.394&	0.075&	0.166&	0.096&  0.710&	0.882&	0.974 \\
			\rowcolor{mygray}
			Model 3&\color{myblue} \textbf{0.389}&	\color{myblue} \textbf{0.070}&\color{myblue} \textbf{0.161}&\color{myblue}\textbf{0.093}& \color{myblue} \textbf{0.718}&	\color{myblue} \textbf{0.890}&	\color{myblue} \textbf{0.976} \\
			% \rowcolor{mygray}
			Model 4 &0.400&	0.078&	0.171&	0.102&  0.700&	0.871&	0.972 \\
			\hline
			\hline
			Model 5 &0.368&0.060&0.147&0.082& 0.739&  0.904 & 0.980\\
			Model 6 &0.362&0.056&0.143&0.078& 0.745&  0.912 & 0.980\\
			Model 7 &0.358&0.054&0.140&0.076& 0.748&  0.917 & 0.982\\
			Model 8 &0.355&0.052&0.137&0.075& 0.752&  0.922 & 0.982\\
			Model 9 &0.356&0.052&0.138&0.074& 0.750&  0.921 & 0.981\\
			\rowcolor{mygray}
			Model 10 & \color{reda} \textbf{0.343}& \color{reda} \textbf{0.048}& \color{reda} \textbf{0.120}& \color{reda} \textbf{0.068}& \color{reda} \textbf{0.763}& \color{reda} \textbf{0.931}  & \color{reda} \textbf{0.984}\\
			Model 11 &0.372&0.064&0.150&0.085& 0.734&  0.900 & 0.978\\
			Model 12 &0.387&0.072&	0.170&	0.105&  0.720&	0.874&	0.973 \\
			\bottomrule[1.5pt]
		\end{tabular}

==> MMFT-TIP(2)/table/ablation_study_rgbd_sod.tex <==
\begin{tabular}{c|c|c|ccccc|ccccc|ccccc|ccccc|ccccc}
			\toprule[1.5pt]
			\multicolumn{1}{c|}{\multirow{2}*{Method}}&\multicolumn{2}{c|}{\emph{}} &\multicolumn{5}{c|}{\emph{SIP}}&\multicolumn{5}{c|}{\emph{STERE}}&\multicolumn{5}{c|}{\emph{NJUD}}&\multicolumn{5}{c|}{\emph{NLPR}}&\multicolumn{5}{c}{\emph{LFSD}}\\
			
			\cmidrule(r){2-3} \cmidrule(r){4-8} \cmidrule(r){9-13} \cmidrule(r){14-18} \cmidrule(r){19-23} \cmidrule(r){24-28} 
			& Params (MB)$\downarrow$ & FLOPs (GB)$\downarrow$ & $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$
			& $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$ 
			& $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$
			& $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$& $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$ \\
			\midrule[1pt]
			
			
			Model 1 & 53.54& 	17.98&  0.860& 	0.766& 	0.831 &	0.833 &	0.062 &	0.868 &	0.784 &	0.849 &	0.862 &	0.051 &	0.872&	0.799&	0.858&	0.847&	0.056&	0.873 &	0.810 &	0.874 &	0.882 	&0.038 &	0.800& 	0.713& 	0.777 &	0.801 &	0.117 
			\\
			% \rowcolor{mygray}
			Model 2 & 55.54&	21.35& 0.884  & 	0.801  & 	0.857 &  	0.863  & 	0.054  & 	0.890  & 	0.817 &  	0.873  & 	0.881  & 	0.044  & 	0.888 & 	0.834 & 	0.878 & 	0.872 & 	0.047	 & 0.890  & 	0.827  & 	0.885  & 	0.899  & 	0.034  & 	0.827  & 	0.741  & 	0.804  & 	0.829  & 	0.105 
			\\
			\rowcolor{mygray}
			Model 3 & 57.54& 24.71& \color{myblue} \textbf{0.896}&	\color{myblue} \textbf{0.812}&	\color{myblue} \textbf{0.866}&	\color{myblue} \textbf{0.874}&	\color{myblue} \textbf{0.051}&	\color{myblue} \textbf{0.899}&	\color{myblue} \textbf{0.830}&	\color{myblue} \textbf{0.887}&	\color{myblue} \textbf{0.895}&	\color{myblue} \textbf{0.042}& \color{myblue} \textbf{0.893}&	\color{myblue} \textbf{0.846}&	\color{myblue} \textbf{0.888}&	\color{myblue} \textbf{0.892}&	\color{myblue} \textbf{0.044}&	\color{myblue} \textbf{0.896}&	\color{myblue} \textbf{0.840}&	\color{myblue} \textbf{0.894}&	\color{myblue} \textbf{0.910}&	\color{myblue} \textbf{0.032}&\color{myblue} \textbf{0.840} &	\color{myblue} \textbf{0.762} &	\color{myblue} \textbf{0.819} &	\color{myblue} \textbf{0.840} &	\color{myblue} \textbf{0.099} 
			\\
			% \rowcolor{mygray}
			Model 4 & 56.62& 23.28& 0.887 &	0.787 &	0.853 &	0.854 &	0.056&	0.887 &	0.814 &	0.877 &	0.883&	0.044 &	0.884&	0.832&	0.880&	0.878&	0.046&	0.890 &	0.823 	&0.883 &	0.896 	&0.035 &	0.818&	0.726&	0.796&	0.831	&0.108
			
			\\
			
			\toprule[1pt]
			\toprule[1pt]
			Model 5 & 60.30&	24.89& 0.910 &	0.841& 	0.882 &	0.901 &	0.046 &	0.911 &	0.855 &	0.900 &	0.916 &	0.038 &	0.910 &	0.869& 	0.902& 	0.911 &	0.038 	&0.909 &	0.860 &	0.911 &	0.932 &	0.028 &	0.851 &	0.792& 	0.834& 	0.855 &	0.083 
			\\
			Model 6 & 63.94&	25.12& 0.913 &	0.850 &	0.886 &	0.909 &	0.044 &	0.917 &	0.866 &	0.907 &	0.928 &	0.037 &	0.918 &	0.882 &	0.908& 	0.923 &	0.036 	&0.912 &	0.867 &	0.915 &	0.940 &	0.027 &	0.856 &	0.799 &	0.838& 	0.862 &	0.080 
			\\
			Model 7 & 71.22&	25.58&0.918 &	0.857 &	0.893 &	0.917 &	0.043 &	0.921 &	0.872 &	0.908 &	0.936 &	0.036 &	0.924 &	0.882 &	0.915 &	0.930& 	0.036 	&0.918 &	0.873 &	0.920 &	0.944 &	0.026 &	0.864 &	0.808 &	0.846 &	0.874 &	0.075 
			\\
			Model 8 & 78.51&	26.05& 0.920 &	0.863 &	0.897 	&0.920 &	0.042 &	0.924 &	0.879& 	0.912 &	0.943 &	0.035 &	0.928 &	0.886 &	0.917 &	0.935 &	0.034 	&0.921 &	0.879 	&0.922 	&0.950 &	0.024& 	0.872 &	0.811 &	0.852& 	0.883 &	0.072 
			\\
			Model 9 & 85.79&	26.52& 0.917 &	0.863 &	0.895 &	0.919 &	0.042 &	0.924 &	0.878 &	0.912 &	0.942 &	0.035 &	0.929 &	0.884 &	0.913 &	0.934 &	0.034 	&0.921 &	0.880 	&0.920 &	0.949& 	0.024& 	0.872 &	0.808 &	0.854 &	0.884 &	0.072 
			\\
			\rowcolor{mygray}
			Model 10  & 75.96&	25.89& \color{reda} \textbf{0.931}&	\color{reda} \textbf{0.881}&	\color{reda} \textbf{0.909}&	\color{reda} \textbf{0.943}&	\color{reda} \textbf{0.038}&	\color{reda} \textbf{0.935}&	\color{reda} \textbf{0.894}&	\color{reda} \textbf{0.925}&	\color{reda} \textbf{0.953}&	\color{reda} \textbf{0.031} &\color{reda} \textbf{0.940}	&\color{reda} \textbf{0.905}&	\color{reda} \textbf{0.927}&	\color{reda} \textbf{0.950}&	\color{reda} \textbf{0.031}&	\color{reda} \textbf{0.931}&	\color{reda} \textbf{0.893}&	\color{reda} \textbf{0.933}&	\color{reda} \textbf{0.958}&	\color{reda} \textbf{0.022} & \color{reda} \textbf{0.897}& 	\color{reda} \textbf{0.843} &	\color{reda} \textbf{0.877} &	\color{reda} \textbf{0.909} &	\color{reda} \textbf{0.063} 
			\\
			% \rowcolor{mygray}
			Model 11 & 76.20&	26.12&  0.908 &	0.852 &	0.883 &	0.907 &	0.045 &	0.921 &	0.870 &	0.913 &	0.932 &	0.037 	&0.917& 	0.877 &	0.916 &	0.921 &	0.037 	&0.911 &	0.870 &	0.913 &	0.937& 	0.028 &	0.855 &	0.803 &	0.835 	&0.857 	&0.080 
			\\
			Model 12 & 76.40&	27.45&  0.894 &	0.808 &	0.868 &	0.879 &	0.052&	0.901 &	0.834 &	0.893 &	0.899 &	0.042 &	0.890 &	0.844 &	0.889 &	0.891 &	0.045 	&0.898 &	0.848& 	0.896 &	0.914 &	0.031 &	0.833 &	0.754 &	0.813& 	0.840 &	0.102 
			\\
			\bottomrule[1.5pt]
		\end{tabular}

==> MMFT-TIP(2)/table/ablation_study_salient_contour.tex <==

		\begin{tabular}{c|cc|cc|cc|cc|cc}
			\toprule[1.5pt]
			\multicolumn{1}{c|}{\multirow{2}*{Method}} &\multicolumn{2}{c|}{\emph{STERE}}&\multicolumn{2}{c|}{\emph{NJUD}}&\multicolumn{2}{c|}{\emph{NLPR}}&\multicolumn{2}{c|}{\emph{SIP}}&\multicolumn{2}{c}{\emph{LFSD}}\\
			
			\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11}  
			&
			$F_{\beta}^{max}\uparrow$   & $\mathcal{M}\downarrow$
			& $F_{\beta}^{max}\uparrow$   & $\mathcal{M}\downarrow$ 
			& $F_{\beta}^{max}\uparrow$   & $\mathcal{M}\downarrow$   
			& $F_{\beta}^{max}\uparrow$   & $\mathcal{M}\downarrow$  
			& $F_{\beta}^{max}\uparrow$   & $\mathcal{M}\downarrow$
			
			\\
			\midrule[1pt]
			% HAINet &	0.532&	0.009&  0.556&	0.011&	0.496&	0.008&  0.428&	0.009&	0.455&	0.018\\
			Model 1  &0.414&0.021&0.432&0.019&0.381&0.019&0.332&0.019&0.393&0.026\\
			Model 2 &0.436&0.018&0.450&0.021&0.400&0.017&0.348&0.017&0.410&0.023\\
			\rowcolor{mygray}
			Model 3 & \color{myblue} \textbf{0.442}&\color{myblue} \textbf{0.018}&\color{myblue} \textbf{0.459}&\color{myblue} \textbf{0.020}&\color{myblue} \textbf{0.406}&\color{myblue} \textbf{0.016}&\color{myblue} \textbf{0.356}&\color{myblue} \textbf{0.016}&\color{myblue} \textbf{0.417}&\color{myblue} \textbf{0.022}\\
			Model 4  &0.430&0.019&0.448&0.022&0.394&0.018&0.340&0.018&0.405&0.023
			\\
			\hline
			\hline
			Model 5&0.454&0.016&0.472&0.018&0.420&0.015&0.366&0.017&0.437&0.020\\
			Model 6&0.460&0.017&0.477&0.019&0.422&0.015&0.372&0.016&0.440&0.019\\
			Model 7&0.465&0.018&0.479&0.019&0.427&0.014&0.380&0.017&0.442&0.019\\
			Model 8&0.468&0.018&0.484&0.019&0.430&0.014&0.385&0.017&0.445&0.019
			\\
			Model 9 &0.466&0.018&0.484&0.019&0.429&0.014&0.386&0.017&0.444&0.019
			\\
			\rowcolor{mygray}
			Model 10 &	 \color{reda} \textbf{0.480}&	 \color{reda} \textbf{0.016}& 	 \color{reda} \textbf{0.494}&	 \color{reda} \textbf{0.017}&	 \color{reda} \textbf{0.443}&	\color{reda} \textbf {0.012}&	 \color{reda} \textbf {0.394}&	 \color{reda} \textbf{0.015}&	 \color{reda} \textbf{0.459}&	 \color{reda} \textbf{0.017}\\
			Model 11&0.459&0.017&0.470&0.019&0.418&0.018&0.364&0.017&0.430&0.020\\
			Model 12 &0.440&0.018&0.457&0.020&0.406&0.017&0.350&0.017&0.417&0.022\\
			
			\bottomrule[1.5pt]
		\end{tabular}

==> MMFT-TIP(2)/table/contour_performance.tex <==

		\begin{tabular}{c|c|cc|cc|cc|cc|cc}
			\toprule[1.5pt]
			\multicolumn{1}{c|}{\multirow{2}*{Method}}&\multicolumn{1}{c|}{\multirow{2}*{Backbone}} &\multicolumn{2}{c|}{\emph{STERE}}&\multicolumn{2}{c|}{\emph{NJUD}}&\multicolumn{2}{c|}{\emph{NLPR}}&\multicolumn{2}{c|}{\emph{SIP}}&\multicolumn{2}{c}{\emph{LFSD}}\\
			
			\cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10} \cmidrule(r){11-12}  
			& &
			$F_{\beta}^{max}\uparrow$   & $\mathcal{M}\downarrow$
			& $F_{\beta}^{max}\uparrow$   & $\mathcal{M}\downarrow$ 
			& $F_{\beta}^{max}\uparrow$   & $\mathcal{M}\downarrow$   
			& $F_{\beta}^{max}\uparrow$   & $\mathcal{M}\downarrow$  
			& $F_{\beta}^{max}\uparrow$   & $\mathcal{M}\downarrow$
			
			\\
			\midrule[1pt]
			% HAINet &	0.532&	0.009&  0.556&	0.011&	0.496&	0.008&  0.428&	0.009&	0.455&	0.018\\
			RD3D~\cite{RD3D} & ResNet-50 & 0.446&	0.017&  0.480&	0.019&	0.435& {0.014}&  0.390&	0.017&	0.440&	0.019 \\
			SPNet~\cite{SPNet} &	Res2Net-50 & 0.393&	0.018 &  0.490&	0.018&	0.426&	0.014&  0.384&	0.018&	0.377&	0.022    \\
			% \rowcolor{myred}
			%  \multicolumn{1}{>{\columncolor{myred}}c}{\color{white}{0.437}}
			\rowcolor{mygray}
			MMFT & ResNet-50&	\color{reda} \textbf{0.493}&	 {0.017}&   \color{reda} \textbf{0.501}&	 \color{reda} \textbf{0.017}&	 \color{reda} \textbf{0.452}& {0.013}& \color{reda} \textbf{0.407}&{0.016}&	 \color{reda} \textbf{0.473}&{0.024}\\
			\rowcolor{mygray}
			MMFT & Res2Net-50&{0.480}&	 \color{reda} \textbf{0.016}& {0.494}&	 \color{reda} \textbf{0.017}&{0.443}&	\color{reda} \textbf {0.012}& {0.394}&	 \color{reda} \textbf{0.015}&{0.459}&	 \color{reda} \textbf{0.017}\\
			
			\bottomrule[1.5pt]
		\end{tabular}

==> MMFT-TIP(2)/table/depth_applying_other_methods.tex <==
\begin{tabular}{c|ccccc|ccccc|ccccc|ccccc|ccccc}
			\toprule[1.5pt]
			\multicolumn{1}{c|}{\multirow{2}*{Method}} &\multicolumn{5}{c|}{\emph{SIP}}&\multicolumn{5}{c|}{\emph{STERE}}&\multicolumn{5}{c|}{\emph{NJUD}}&\multicolumn{5}{c|}{\emph{NLPR}}&\multicolumn{5}{c}{\emph{LFSD}}\\
			
			\cmidrule(r){2-6} \cmidrule(r){7-11} \cmidrule(r){12-16} \cmidrule(r){17-21} \cmidrule(r){22-26} 
			& $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$
			& $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$ 
			& $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$
			& $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$ 
			& $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$ 
			\\
			\midrule[1pt]
			
			
			Two-stream FPN$\ast$ & 0.886&	0.810&	0.847&	0.890&	0.061&	0.882&	0.815&	0.865& {0.899}&	0.051& 0.893&	0.834&	0.868&	0.901&	0.052&	0.896&	0.845&	0.889&	0.920&	0.035 &0.844 &	0.767 &	0.827 &	0.864 &	0.098 \\
			\rowcolor{mygray}
			Two-stream FPN$\ddagger$& \color{reda} \textbf{0.903}&	\color{reda} \textbf{0.840}&	\color{reda} \textbf{0.881}&	\color{reda} \textbf{0.919}&	\color{reda} \textbf{0.045}&	\color{reda} \textbf{0.911}&	\color{reda} \textbf{0.850}&	\color{reda} \textbf{0.890}&	\color{reda} \textbf{0.914}&	\color{reda} \textbf{0.042}& \color{reda} \textbf{0.909}&	\color{reda} \textbf{0.857}&	\color{reda} \textbf{0.894}&	\color{reda} \textbf{0.921}&	\color{reda} \textbf{0.043}&	\color{reda} \textbf{0.914}&	\color{reda} \textbf{0.859}&	\color{reda} \textbf{0.918}&	\color{reda} \textbf{0.945}&	\color{reda} \textbf{0.029} 
			&\color{reda} \textbf{0.855} &	\color{reda} \textbf{0.787} &	\color{reda} \textbf{0.839} &	\color{reda} \textbf{0.880} &	\color{reda} \textbf{0.088} 
			\\
			RD3D$\ast$~\cite{RD3D} & 0.906 &	0.845 &	0.885 &	0.924 &	0.048&  0.917 &	0.871& 	0.911 &	0.944& 	0.037 
			&0.923 	&0.886 	&0.916 	&0.942 &	0.037 &0.927 	&0.889 &	0.929 &	\color{reda} \textbf{0.959} &	0.022 &0.879 &	0.816 &	0.858 &	0.898 &	0.073 
			\\
			\rowcolor{mygray}
			RD3D$\ddagger$~\cite{RD3D} & \color{reda} \textbf{0.925} &	\color{reda} \textbf{0.879} &	\color{reda} \textbf{0.905} &	\color{reda} \textbf{0.940} &	\color{reda} \textbf{0.038} &	\color{reda} \textbf{0.932} &	\color{reda} \textbf{0.893} &	\color{reda} \textbf{0.922} &	\color{reda} \textbf{0.948} &	\color{reda} \textbf{0.030} &\color{reda} \textbf{0.937} &	\color{reda} \textbf{0.902} &	\color{reda} \textbf{0.924} &	\color{reda} \textbf{0.947} &	\color{reda} \textbf{0.031} &	\color{reda} \textbf{0.928} &	\color{reda} \textbf{0.893} &	\color{reda} \textbf{0.929} &	{0.957} & \color{reda} \textbf{0.022}&	\color{reda} \textbf{0.888} &	\color{reda} \textbf{0.828} &	\color{reda} \textbf{0.867} &	\color{reda} \textbf{0.898} & \color{reda} \textbf{0.068}\\
			SPNet$\ast$~\cite{SPNet} &0.916 &	0.868 &	0.894 	&0.931 	&0.043 &0.915 &	0.873 &	0.907 &	0.942 	&0.037 &0.935 &	0.906 	&0.924 	&0.953 &	0.029  &0.926 &	0.896 &	0.927 	&0.959 &	0.021 &0.881 &	0.823 &	0.854 &	0.897 	&0.071 
			
			\\
			\rowcolor{mygray}
			SPNet$\ddagger$~\cite{SPNet}& \color{reda} \textbf{0.928}&	\color{reda} \textbf{0.883}&	\color{reda} \textbf{0.907}&	\color{reda} \textbf{0.942}&	\color{reda} \textbf{0.037}&	\color{reda} \textbf{0.931}&	\color{reda} \textbf{0.894}&	\color{reda} \textbf{0.922}&	\color{reda} \textbf{0.952}&	\color{reda} \textbf{0.030}& \color{reda} \textbf{0.941}&	\color{reda} \textbf{0.910}&	\color{reda} \textbf{0.928}&	\color{reda} \textbf{0.954}&	\color{reda} \textbf{0.029}&	\color{reda} \textbf{0.931}&	\color{reda} \textbf{0.898}&	\color{reda} \textbf{0.930}&	\color{reda} \textbf{0.961}&	\color{reda} \textbf{0.021} &	\color{reda} \textbf{0.882}&	\color{reda} \textbf{0.826}&	\color{reda} \textbf{0.866}&	\color{reda} \textbf{0.901}&	\color{reda} \textbf{0.065}\\
			% JL-DCF\ast& 0.924&	0.863&	0.905&	0.938&	0.043&	0.913&	0.857&	0.903&	0.937&	0.040& 0.912&	0.869&	0.902&	0.935&	0.041&	0.925&	\color{reda} \textbf{0.882}&	0.925&	\color{reda} \textbf{0.955}&	\color{reda} \textbf{0.022} \\
			%  \rowcolor{mygray}
			% JL-DCF\ddagger  &\color{reda} \textbf{0.948}&	\color{reda} \textbf{0.909}&	\color{reda} \textbf{0.930}&	\color{reda} \textbf{0.959}&	\color{reda} \textbf{0.028}&	\color{reda} \textbf{0.921}&	\color{reda} \textbf{0.870}&	\color{reda} \textbf{0.916}&	\color{reda} \textbf{0.944}&	\color{reda} \textbf{0.037}& \color{reda} \textbf{0.918}&	\color{reda} \textbf{0.874}&	\color{reda} \textbf{0.911}&	\color{reda} \textbf{0.936}&	\color{reda} \textbf{0.040}&	\color{reda} \textbf{0.925}&	0.878&	\color{reda} \textbf{0.928}&	0.953&	0.023 \\
			\bottomrule[1.5pt]
		\end{tabular}

==> MMFT-TIP(2)/table/depth_estimation_performance.tex <==
\begin{tabular}{c|c|cccc|ccc}
			\toprule[1.5pt]
			\multicolumn{1}{c|}{\multirow{2}*{Method}} &\multicolumn{1}{c|}{\multirow{2}*{Backbone}} &\multicolumn{4}{c|}{{Error}} & \multicolumn{3}{c}{{Accuracy}}\\
			
			\cmidrule(r){3-6} \cmidrule(r){7-9} 
			&& RMSE $\downarrow$   & RMSE (log) $\downarrow$
			& Abs Rel $\downarrow$   & Sq ReL $\downarrow$ & P1 $\uparrow$   & P2 $\uparrow$   
			& P3 $\uparrow$   
			\\
			\midrule[1pt]
			DASNet~\cite{DASNet} & ResNet-50&0.378&0.053&	0.130&	0.078& 0.739&	0.920&	0.984 \\
			CoNet~\cite{CoNet} & ResNet-101&0.433&0.062&	0.149&	0.094& 0.677&	0.907&	0.984 \\
			% FCRN & 66.901&	1.090&	3.018&	273.43 &0.444&  0.345&	0.521&	0.619 \\
			TL-Depth~\cite{TL-Depth} & ResNet-101&0.387&0.056&	0.134&	0.081& 0.721&	0.911&	0.983 \\
			LAP-Depth~\cite{LAP-Depth} & ResNet-101&0.404&0.049&	 {0.155}&	{0.111}& \color{reda} \textbf{0.771}&  0.925&	0.982 \\
			\rowcolor{mygray}
			MMFT &ResNet-50& \color{reda} \textbf{0.353} & \color{reda} \textbf{0.049}&	\color{reda} \textbf {0.124}& \color{reda} \textbf{0.070}&   {0.749}&  \color{reda} \textbf{0.931}&	 \color{reda} \textbf{0.986}\\
			\rowcolor{mygray}
			MMFT &ResNet-101& {0.355} & {0.050}&	 \color{reda} \textbf{0.124}&{0.071}&   {0.750}&  {0.927}&	 {0.985}\\
			\bottomrule[1.5pt]
		\end{tabular}

==> MMFT-TIP(2)/table/param_flops.tex <==

 \begin{tabular}{r||cccccccccccccc}
\toprule[1.5pt]
% \rowcolor{mygray}
		Model Nmae  &{CDNet$_{21}$} &{DFMNet$_{21}$} &{DSA2F$_{21}$} &{DCF$_{21}$}&{HAINet$_{21}$} &   {RD3D$_{21}$} &   {SPNet$_{21}$} & {A2DELE$_{20}$}&{DASNet$_{20}$}&{CoNet$_{20}$} & {MMFT} &{MMFT} & {MMFT} & {MMFT} \\
		% \rowcolor{mygray}
&~\cite{CDNet}&~\cite{DFMNet}&~\cite{DSA2F}&~\cite{DCF}&~\cite{HAINet}&~\cite{RD3D}&~\cite{SPNet}&~\cite{A2DELE}&~\cite{DASNet}&~\cite{CoNet}& \\
		% \rowcolor{mygray}
		Backbone  &VGG-16 &ResNet-34& VGG-19& ResNet-50& VGG-16& ResNet-50& Res2Net-50&  VGG-16& ResNet-50&ResNet-101& VGG-16& ResNet-50& Res2Net-50& ResNet-101 \\
	\midrule[1pt]
		Parameters (MB)$\downarrow$    & \color{myblue}\textbf{32.93} &\color{mygreen}\textbf{23.44} & 36.48 & {47.85} & 59.82 &{46.90}&\textbf{150.31}&\color{reda}\textbf{14.90}&{36.68}&43.66& {41.38}&53.12&{75.96}&72.13
		\\
		FLOPs (G)$\downarrow$     &{72.10} & 26.32 &{172.23} &\color{reda}\textbf{17.74} & \textbf{181.41} & 50.72 &{67.92}&39.07&{28.56}&{27.37}&72.82&\color{mygreen}\textbf{20.32}&25.89&\color{myblue}\textbf{25.50}
		\\
 \bottomrule[1.5pt]
	\end{tabular}


==> MMFT-TIP(2)/table/param_flops_response.tex <==

 \begin{tabular}{r||cccccccccccccc}
\toprule[1.5pt]
% \rowcolor{mygray}
		Model Nmae  &{CDNet$_{21}$} &{DFMNet$_{21}$} &{DSA2F$_{21}$} &{DCF$_{21}$}&{HAINet$_{21}$} &   {RD3D$_{21}$} &   {SPNet$_{21}$} & {A2DELE$_{20}$}&{DASNet$_{20}$}&{CoNet$_{20}$} & {MMFT} &{MMFT} & {MMFT} & {MMFT} \\
		Backbone  &VGG-16 &ResNet-34& VGG-19& ResNet-50& VGG-16& ResNet-50& Res2Net-50&  VGG-16& ResNet-50&ResNet-101& VGG-16& ResNet-50& Res2Net-50& ResNet-101 \\
	\midrule[1pt]
		Parameters (MB)$\downarrow$    & \color{myblue}\textbf{32.93} &\color{mygreen}\textbf{23.44} & 36.48 & {47.85} & 59.82 &{46.90}&\textbf{150.31}&\color{reda}\textbf{14.90}&{36.68}&43.66& {41.38}&53.12&{75.96}&72.13
		\\
		FLOPs (G)$\downarrow$     &{72.10} & 26.32 &{172.23} &\color{reda}\textbf{17.74} & \textbf{181.41} & 50.72 &{67.92}&39.07&{28.56}&{27.37}&72.82&\color{mygreen}\textbf{20.32}&25.89&\color{myblue}\textbf{25.50}
		\\
 \bottomrule[1.5pt]
	\end{tabular}


==> MMFT-TIP(2)/table/rgb_sod_performance.tex <==
	\begin{tabular}{c|c|c|ccccc|ccccc|ccccc|ccccc|ccccc}
			\toprule[1.5pt]
			\multicolumn{1}{c|}{\multirow{2}*{Method}}&\multicolumn{1}{c|}{\multirow{2}*{Publication}}&\multicolumn{1}{c|}{\multirow{2}*{Backbone}} &\multicolumn{5}{c|}{\emph{DUTS}}&\multicolumn{5}{c|}{\emph{DUT-OMRON}}&\multicolumn{5}{c|}{\emph{ECSSD}}&\multicolumn{5}{c|}{\emph{HKU-IS}}&\multicolumn{5}{c}{\emph{PASCAL-S}}\\
			
			\cmidrule(r){4-8} \cmidrule(r){9-13} \cmidrule(r){14-18} \cmidrule(r){19-23} \cmidrule(r){24-28} 
			&& & $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$
			& $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$ 
			& $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$
			& $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$& $F_{\beta}^{max}\uparrow$  & $F_{\beta}^{w}\uparrow$ &  $S_m\uparrow $ &  $E_m\uparrow $ & $\mathcal{M}\downarrow$ \\
			\midrule[1pt]
			
			GateNet~\cite{GateNet}&ECCV 2020 & ResNet-50&0.888 	&0.809 	&0.884 &	0.903 &	0.040 &	0.818 &	0.729 	&0.837 &	0.868 &	0.055 &	0.945 &	0.894 &	0.920 	&0.943 	&0.040 &	0.933 &	0.881 &	0.915 &	0.954 	&0.033 &	0.881 &	0.804& 	0.854 &	0.882 &	0.071 
			\\
			% \rowcolor{mygray}
			ITSD~\cite{ITSD} &CVPR 2020& ResNet-50 &0.883 &	0.824 &	0.883 &	0.898 	&0.041 &	0.821 &	0.750 &	0.839 &	0.867 &	0.061 	&0.947 &	0.911 &	0.925 &	0.932 &	0.035 &	0.933 	&0.893 &	0.916 &	0.953 &	0.031 &	0.882 &	0.823 	&0.859 	&0.866 &	0.066 
			
			\\
			MINet~\cite{MINet} &CVPR 2020& ResNet-50&0.884 	&0.825& 	0.883 &	0.917 	&\color{myblue} \textbf{0.037} &	0.810 &	0.738 &	0.832 &	0.873 &	0.056 	&0.948 &	0.911 &	0.925 &	0.953 &	0.034 &	0.935 	&0.899 &	0.919 	&\color{mygreen} \textbf{0.961} &	\color{mygreen} \textbf{0.028} &	0.880 &	0.818 	&0.854 &	0.897& 	0.066 
			
			\\
			% \rowcolor{mygray}
			GCPA~\cite{GCPA} & AAAI 2020& ResNet-50&0.888 &	0.821 &	0.889 &	0.913 	&0.038 &	0.812 &	0.734 &	0.837 &	0.869 &	0.056 	&0.949 &	0.903 &	0.927 &	0.952 &	0.035& 	0.939 	&0.889 	&\color{myblue} \textbf{0.920} &	0.956 &	0.032 &	0.882 &	0.819 	&\color{mygreen} \textbf{0.864} &	0.899 &	0.064 
			\\
			F3Net~\cite{F3Net} &AAAI 2020 & ResNet-50&	0.891 &		0.835 &		0.887 &		0.918 	&	\color{mygreen} \textbf{0.035} &		0.813 &		0.747 &		0.837 &		0.876 &		0.053 	&	0.945 &		0.912 &		0.924 &		0.946 &		\color{myblue} \textbf{0.033} &		0.937 	&	0.900 &		0.916 &		0.959 	&	\color{mygreen} \textbf{0.028} &		0.882 &		0.823 	&	0.857 &		0.892 &		0.064 
			
			\\
			VST~\cite{VST}&ICCV 2021&T2T~\cite{T2T}&0.890 &	0.828 &	\color{reda} \textbf{0.895} &	0.916 	&\color{myblue} \textbf{0.037} &	\color{myblue} \textbf{0.825} &	0.755 &	\color{reda} \textbf{0.849} &	0.872 &	0.058 	&\color{myblue} \textbf{0.951} &	0.910 &	\color{mygreen} \textbf{0.932} &\color{mygreen} \textbf{0.957} &	\color{myblue} \textbf{0.033} &	\color{mygreen} \textbf{0.942} 	&0.898 &	\color{reda} \textbf{0.928} &	\color{mygreen} \textbf{0.961} &	\color{myblue} \textbf{0.029} 	&\color{mygreen} \textbf{0.890} &	0.827 	&\color{reda} \textbf{0.871} &\color{reda} \textbf{0.905} &	\color{myblue} \textbf{0.062} 
			
			\\
			SAMNet~\cite{SAMNet} &TIP 2021&SAM~\cite{SAMNet}&\color{myblue} \textbf{0.894} &	0.840 &	0.890 &	\color{myblue} \textbf{0.923} 	&\color{mygreen} \textbf{0.035} &	0.823 &	\color{myblue} \textbf{0.760} 	&\color{myblue} \textbf{0.844} &	\color{myblue} \textbf{0.885} &	\color{myblue} \textbf{0.051} 	&\color{mygreen} \textbf{0.952}& 	\color{mygreen} \textbf{0.920} &	\color{myblue} \textbf{0.928} &	\color{reda} \textbf{0.958} &	\color{mygreen} \textbf{0.032} &	\color{myblue} \textbf{0.940} 	&\color{reda} \textbf{0.905} &	\color{mygreen} \textbf{0.921} &	\color{reda} \textbf{0.963} &	\color{reda} \textbf{0.027} &	\color{myblue} \textbf{0.887} &	\color{myblue} \textbf{0.832} 	&\color{myblue} \textbf{0.862} &\color{myblue} \textbf{0.903} &	\color{myblue} \textbf{0.062} 
			
			\\
			Auto-MSFNet~\cite{Auto-MSFNet}&ACMMM 2021&ResNet-50 &0.877 &	\color{myblue} \textbf{0.841} &	0.876 	&\color{reda} \textbf{0.931} &	\color{reda} \textbf{0.034}& 	0.798 &	0.757 &	0.831 &	0.876 	&\color{mygreen} \textbf{0.050} &	0.941 &	\color{myblue} \textbf{0.916} &	0.914 &	\color{myblue} \textbf{0.954} &	\color{myblue} \textbf{0.033} 	&0.928 &	\color{mygreen} \textbf{0.904}& 	0.908 &	\color{myblue} \textbf{0.960} &	\color{reda} \textbf{0.027} &	0.877 	&\color{mygreen} \textbf{0.834} &	0.851 &	\color{reda} \textbf{0.905} &	\color{mygreen} \textbf{0.061} 
			
			\\
			SGL-KRN~\cite{SGL-KRN} &AAAI 2021&ResNet-50 &\color{mygreen} \textbf{0.898} 	&\color{reda} \textbf{0.847} 	&\color{myblue} \textbf{0.891} &	\color{mygreen} \textbf{0.926} 	&\color{reda} \textbf{0.034} &	\color{mygreen} \textbf{0.827}& 	\color{mygreen} \textbf{0.765} &	\color{mygreen} \textbf{0.845} &	\color{mygreen} \textbf{0.889} &\color{reda} \textbf{0.049} 	&0.946 &	0.910 &	0.923 &	0.942 &	0.036 &	0.937 	&\color{myblue} \textbf{0.902} &	0.918 &	\color{myblue} \textbf{0.960} &	\color{myblue} \textbf{0.029}& 	\color{myblue} \textbf{0.887} &	0.826 	&0.856 &	0.883 &	0.068
			\\
			\midrule[1pt]
			\rowcolor{mygray}
			\multicolumn{2}{c|}{\multirow{1}*{Ours}}&ResNet-50&\color{reda} \textbf{0.904} &	\color{mygreen} \textbf{0.844} 	&\color{mygreen} \textbf{0.893} 	&\color{reda} \textbf{0.931} &	\color{reda} \textbf{0.034} &	\color{reda} \textbf{0.831} &	\color{reda} \textbf{0.766} &	\color{reda} \textbf{0.849} 	&\color{reda} \textbf{0.893} &	\color{reda} \textbf{0.049} &	\color{reda} \textbf{0.960} 	&\color{reda} \textbf{0.925} 	&\color{reda} \textbf{0.936} &\color{reda} \textbf{0.958} 	&\color{reda} \textbf{0.029} &	\color{reda} \textbf{0.944}& 	0.901& 	\color{mygreen} \textbf{0.921} &	\color{mygreen} \textbf{0.961} 	&\color{myblue} \textbf{0.029} &	\color{reda} \textbf{0.894}& 	\color{reda} \textbf{0.837} &	\color{reda} \textbf{0.871}& 	\color{mygreen} \textbf{0.904} &\color{reda} \textbf{0.059} 
			
			\\
			\bottomrule[1.5pt]
		\end{tabular}

==> MMFT-TIP(2)/table/rgbd_sod_performance.tex <==
\begin{tabular}{cr||cccccccccccccccc||ccc>{\columncolor{mygray}}c>{\columncolor{mygray}}c>{\columncolor{mygray}}c>{\columncolor{mygray}}c}
			\toprule[2pt]
			\multicolumn{2}{l||}{} & \multicolumn{16}{c||}{\textbf{{Depth-based Models}}}  & \multicolumn{7}{c}{\textbf{{Depth-free Models}}} \\
			\hline
			\multicolumn{2}{c||}{\multirow{3}{*}{Metric}}   &{S2MA$_{20}$} & {CMWNet$_{20}$} & {BBSNet$_{20}$} & {BBSNet$_{20}$} &{JL-DCF$_{20}$}  & {UCNet$_{20}$} & {PGAR$_{20}$} &{HDFNet$_{20}$}
			&{HDFNet$_{20}$}
			&{CDNet$_{21}$} &{DFMNet$_{21}$} &{DSA2F$_{21}$} &{DCF$_{21}$}&{HAINet$_{21}$} &   {RD3D$_{21}$} &   {SPNet$_{21}$} & {A2DELE$_{20}$}&{DASNet$_{20}$}&{CoNet$_{20}$} & {MMFT} &{MMFT} & {MMFT} & {MMFT} 
			\\
			\multicolumn{2}{l||}{}   & ~\cite{S2MA}&~\cite{CMWNet}&~\cite{BBSNet}&~\cite{BBSNet}&~\cite{JLDCF}&~\cite{UCNet}&~\cite{PGAR}&~\cite{HDFNet}&~\cite{HDFNet}&~\cite{CDNet}&~\cite{DFMNet}&~\cite{DSA2F}&~\cite{DCF}&~\cite{HAINet}&~\cite{RD3D}&~\cite{SPNet}&~\cite{A2DELE}&~\cite{DASNet}&~\cite{CoNet}&\cellcolor{mygray}&\cellcolor{mygray}&\cellcolor{mygray}&\cellcolor{mygray}
			\\
			\multicolumn{2}{l||}{}   & VGG-16  & VGG-16& VGG-16& ResNet-50&ResNet-101& VGG-16& VGG-16&  VGG-16& ResNet-50& VGG-16 &ResNet-34& VGG-19& ResNet-50& VGG-16& ResNet-50& Res2Net-50&  VGG-16& ResNet-50&ResNet-101& VGG-16& ResNet-50& Res2Net-50& ResNet-101
			\\
			% \multicolumn{2}{l|}{}   
			% &  \multicolumn{1}{c}{\Large{~\cite{CTMF}}}         &    \multicolumn{1}{c}{\Large{~\cite{PCA}}}           &   \multicolumn{1}{c}{\Large{~\cite{MMCI}}}           &  \multicolumn{1}{c}{\Large{~\cite{TANet}}}   & \multicolumn{1}{c}{\Large{~\cite{CPFP}}}      &  \multicolumn{1}{c}{\Large{~\cite{DMRA}}}       &   \multicolumn{1}{c}{\Large{~\cite{ICNet}}}    &   \multicolumn{1}{c}{\Large{~\cite{A2DELE}}}     &   \multicolumn{1}{c}{\Large{~\cite{LSSA}}}    &   \multicolumn{1}{c}{\Large{~\cite{DANet}}}    &   \multicolumn{1}{c}{\LARGE{~\cite{CMWNet}}}&   \multicolumn{1}{c}{\LARGE{~\cite{HAINet}}}&   \multicolumn{1}{c}{\LARGE{~\cite{DFM-Net}}}       &  \multicolumn{1}{c|}{}&  \multicolumn{1}{c}{}  \\
			\hline
			% & \Large{CTMF$_{18}$}         & \Large{PCANet$_{18}$}         &\Large{ MMCI$_{19}$} &\Large{TANet$_{19}$} &\Large{CPFP$_{19}$} & \Large{DMRA$_{19}$} & \Large{ICNet$_{20}$} &\Large{A2DELE$_{20}$} & \Large{LSSA$_{20}$} & \Large{DANet$_{20}$} &\Large{CMWNet$_{20}$} &\Large{Ours}  &\Large{Ours} 
			
			% \multicolumn{2}{l|}{}   & \Large{DES$_{14}$}         & \Large{DCMC$_{16}$}         &\Large{ CDCP$_{17}$}     &\Large{DF$_{17}$} &\Large{ CTMF$_{18}$} & \Large{PCANet$_{18}$} & \Large{MMCI$_{19}$} &\Large{TANet$_{19}$} & \Large{CPFP$_{19}$} & \Large{DANet} &\Large{ DMRA$_{19}$} &\Large{DANet}   \\
			
			% \multirow{5}{*}{\emph{\rotatebox{90}{RGBD135}}}      
			% &$F_{\beta}^{max}\uparrow$  
			% &   \multicolumn{1}{c}{\Large{0.877}}  &\multicolumn{1}{c}{\Large{0.925}}  &  \multicolumn{1}{c}{\Large\textbf{0.944}}      &  \multicolumn{1}{c}{\Large{0.916}}      &  \multicolumn{1}{c}{\Large\textbf{0.939}}  &  \multicolumn{1}{c}{\Large{0.923}}  &  \multicolumn{1}{c}{{\Large{0.936}}} &  \multicolumn{1}{c}{\Large{0.926}} &  \multicolumn{1}{c}{\Large{0.934}} &  \multicolumn{1}{c}{\Large\textbf{0.939}}&  \multicolumn{1}{c}{\Large{0.930}}&    \multicolumn{1}{c}{{\Large{0.930}}}  &  \multicolumn{1}{c}{{\Large{0.926}}} &  \multicolumn{1}{c}{{\Large{0.936}}}   &  \multicolumn{1}{c||}{\textbf{\Large{0.944}}}  & \multicolumn{1}{c}{\Large{0.897}}  &  \multicolumn{1}{c}{\Large{0.915}}  &  \multicolumn{1}{c}{\textbf{\Large{0.941}}}     \\
			% &$F_{\beta}^{w}\uparrow$   
			% &   \multicolumn{1}{c}{\Large{0.779}}    &\multicolumn{1}{c}{\Large{0.867}}  &  \multicolumn{1}{c}{\Large{0.892}}      &  \multicolumn{1}{c}{\Large{0.848}}   &  \multicolumn{1}{c}{\Large{0.888}}       &  \multicolumn{1}{c}{\Large{0.845}}     &  \multicolumn{1}{c}{\textbf{\Large{0.908}}}  &    \multicolumn{1}{c}{\Large{0.855}} &  \multicolumn{1}{c}{\Large{0.902}}   &  \multicolumn{1}{c}{\Large{0.894}} &  \multicolumn{1}{c}{\Large{0.888}} &  \multicolumn{1}{c}{{\Large{0.882}}}     &   \multicolumn{1}{c}{{\Large{0.876}}}  &   \multicolumn{1}{c}{{\Large{0.898}}}      &   \multicolumn{1}{c||}{\textbf{\Large{0.917}}} & \multicolumn{1}{c}{\Large{0.836}}    &  \multicolumn{1}{c}{\Large{0.849}}    &   \multicolumn{1}{c}{\textbf{\Large{0.910}}}           \\
			% & $S_m\uparrow$         
			% &   \multicolumn{1}{c}{\Large{0.779}}   
			% &\multicolumn{1}{c}{\Large{0.920}}  &  \multicolumn{1}{c}{\textbf{\Large{0.941}}}      &  \multicolumn{1}{c}{\Large{0.905}}   &  \multicolumn{1}{c}{\textbf{\Large{0.934}}} &  \multicolumn{1}{c}{\Large{0.908}}&  \multicolumn{1}{c}{\textbf{\Large{0.934}}} &  \multicolumn{1}{c}{\Large{0.913}}               &    \multicolumn{1}{c}{\Large{0.932}}&    \multicolumn{1}{c}{\textbf{\Large{0.936}}}&    \multicolumn{1}{c}{\Large{0.931}}&  \multicolumn{1}{c}{{\Large{0.916}}}         &   \multicolumn{1}{c}{{\Large{0.916}}}  &   \multicolumn{1}{c}{{\Large{0.929}}}  &   \multicolumn{1}{c||}{\textbf{\Large{0.936}}} & \multicolumn{1}{c}{\Large{0.886}} &  \multicolumn{1}{c}{\Large{0.909}}   &   \multicolumn{1}{c}{{\Large{0.932}}}        \\
			% & $E_m\uparrow$     
			% &   \multicolumn{1}{c}{\Large{0.923}}   &\multicolumn{1}{c}{\Large{0.959}}  &  \multicolumn{1}{c}{\textbf{\Large{0.974}}}      &  \multicolumn{1}{c}{\Large{0.961}}   &  \multicolumn{1}{c}{\Large{0.967}}      &  \multicolumn{1}{c}{\Large{0.941}}    &  \multicolumn{1}{c}{\textbf{\Large{0.974}}}    &  \multicolumn{1}{c}{\Large{0.939}}  &  \multicolumn{1}{c}{{\Large{0.973}}}  &  \multicolumn{1}{c}{\Large{0.969}}&  \multicolumn{1}{c}{\Large{0.971}} &    \multicolumn{1}{c}{{\Large{0.955}}}    &   \multicolumn{1}{c}{{\Large{0.958}}}    &   \multicolumn{1}{c}{{\Large{0.967}}} &   \multicolumn{1}{c||}{\textbf{\Large{0.978}}}  & \multicolumn{1}{c}{\Large{0.920}}  &  \multicolumn{1}{c}{\Large{0.945}}   &   \multicolumn{1}{c}{\textbf{\Large{0.976}}}    \\
			% &$\mathcal{M}\downarrow$  
			% &   \multicolumn{1}{c}{\Large{0.040}}     &\multicolumn{1}{c}{\Large{0.027}}  &  \multicolumn{1}{c}{\Large{0.021}}      &  \multicolumn{1}{c}{\Large{0.028}}    &  \multicolumn{1}{c}{\Large{0.022}}    &  \multicolumn{1}{c}{\Large{0.029}}     &  \multicolumn{1}{c}{\textbf{\Large{0.019}}} &  \multicolumn{1}{c}{\Large{0.026}}           &    \multicolumn{1}{c}{\textbf{\Large{0.020}}}   &    \multicolumn{1}{c}{\textbf{\Large{0.020}}} &    \multicolumn{1}{c}{\Large{0.021}}  &   \multicolumn{1}{c}{{\Large{0.023}}}   &  \multicolumn{1}{c}{{\Large{0.023}}}  &  \multicolumn{1}{c}{\textbf{\Large{0.019}}}&  \multicolumn{1}{c||}{\textbf{\Large{0.017}}}& \multicolumn{1}{c}{\Large{0.029}} &  \multicolumn{1}{c}{\Large{0.028}}&  \multicolumn{1}{c}{\textbf{\Large{0.019}}}    \\
			\hline
			\multirow{5}{*}{\emph{\rotatebox{90}{DUTLF-D}}}      
			&$F_{\beta}^{max}\uparrow$   
			& 0.909 
			& 0.905 
			& -
			& -
			& 0.924 
			& -
			& 0.938 
			& 0.926 
			& 0.930 
			& 0.901 
			& -
			& 0.938 
			& 0.941 
			& 0.932 
			& 0.946 
			& -
			& 0.907 
			& -
			& 0.935 
			& 0.950 
			& \color{myblue} \textbf{0.955}
			& \color{reda} \textbf{0.958} 
			& \color{mygreen} \textbf{0.956}
			
			\\
			&$F_{\beta}^{w}\uparrow$    
			&  0.862 
			&0.831 
			&-
			&-
			&0.863 
			&-
			&0.889 
			&0.865 
			&0.864 
			&0.838 
			&-
			&0.908 
			&0.909 
			&0.883 
			&0.909 
			&-
			&0.864 
			& -
			&0.891 
			&0.909 
			& \color{myblue} \textbf{0.920} 
			& \color{reda} \textbf{0.926} 
			& \color{mygreen} \textbf{0.924} 
			\\
			& $S_m\uparrow$  
			& 0.903 
			&0.887 
			&-
			&-
			&0.905 
			&-
			&0.920 
			&0.905 
			&0.907 
			&0.886 
			&-
			&0.921 
			&0.924 
			&0.909 
			&0.931 
			&-
			&0.886 
			& -
			&0.919 
			&0.934 
			& \color{myblue} \textbf{0.941} 
			& \color{mygreen} \textbf{0.942} 
			& \color{reda} \textbf{0.943} 
			
			\\
			& $E_m\uparrow$    &
			0.921 
			&0.922 
			&-
			&-
			&0.938 
			&-
			&0.950 
			&0.938 
			&0.938 
			&0.917 
			&-
			&0.956 
			&0.957 
			&0.939 
			&0.957 
			&-
			&0.929 
			& -
			&0.952 
			& \color{myblue} \textbf{0.959} 
			& \color{mygreen} \textbf{0.967} 
			& \color{mygreen} \textbf{0.967} 
			& \color{reda} \textbf{0.968} 
			\\
			&$\mathcal{M}\downarrow$  &   0.044 
			& 0.056 
			& -
			& -
			& 0.043 
			& -
			& 0.035 
			& 0.040 
			& 0.041 
			& 0.051 
			& -
			& 0.031 
			& 0.030 
			& 0.038 
			& 0.031 
			& -
			& 0.043 
			& -
			& 0.033 
			& 0.029 
			& \color{myblue} \textbf{0.027} 
			& \color{mygreen} \textbf{0.025} 
			& \color{reda} \textbf{0.024} 
			\\
				&$AUC\uparrow$ 
&.9721
&.9749
&-
&-
&.9835
&-
&.9802
&\color{mygreen} \textbf{.9892}
&\color{myblue} \textbf{.9884}
&.9567
&-
&.9662
&.9767
&.9777
&.9826
&-
&.9371
&-
&.9817
&.9879
&\color{reda} \textbf{.9893}
&.9856
&.9882

			\\
			\hline
			\multirow{5}{*}{\emph{\rotatebox{90}{STERE}}}      
			&$F_{\beta}^{max}\uparrow$   &   
			0.895 
			& 0.911 
			& 0.901 
			& 0.919 
			& 0.913 
			& 0.908 
			& 0.911 
			& 0.918 
			& 0.910 
			& 0.909 
			& 0.914 
			& 0.910 
			& 0.915 
			& 0.919 
			& 0.917 
			& 0.915 
			& 0.892 
			& 0.915 
			& 0.909 
			& \color{myblue} \textbf{0.931} 
			&  \color{mygreen} \textbf{0.933 }
			&  \color{reda} \textbf{0.935} 
			&  \color{blue} \textbf{0.931} 
			
			\\
			&$F_{\beta}^{w}\uparrow$    &   
			0.825 
			&0.847 
			&0.838 
			&0.858 
			&0.857 
			&0.867 
			&0.856 
			&0.863 
			&0.853 
			&0.855 
			&0.860 
			&0.869 
			&0.873 
			&0.871 
			&0.871 
			&0.873 
			&0.846 
			& 0.872
			&0.866 
			& \color{myblue} \textbf{0.886} 
			& \color{mygreen} \textbf{0.889} 
			& \color{reda} \textbf{0.894} 
			&  \color{mygreen} \textbf{0.889} 
			\\
			& $S_m\uparrow$  &  
			0.890 
			&0.905 
			&0.896 
			&0.908 
			&0.903 
			&0.903 
			&0.907 
			&0.906 
			&0.900 
			&0.903 
			&0.908 
			&0.897 
			&0.905 
			&0.909 
			&0.911 
			&0.907 
			&0.878 
			& 0.910
			&0.905 
			& \color{myblue} \textbf{0.923} 
			& \color{reda} \textbf{0.926} 
			& \color{mygreen} \textbf{0.925} 
			&0.921 
			
			
			\\
			& $E_m\uparrow$    &  
			0.926 
			& 0.930 
			& 0.928 
			& 0.941 
			& 0.937 
			& 0.942 
			& 0.937 
			& 0.937 
			& 0.931 
			& 0.938 
			& 0.939 
			& 0.942 
			& 0.943 
			& 0.938 
			& 0.944 
			& 0.942 
			& 0.928 
			& 0.941
			& 0.941 
			& \color{myblue} \textbf{0.949} 
			& 0.947 
			&  \color{reda} \textbf{0.953} 
			&  \color{mygreen} \textbf{0.952} 
			
			\\
			&$\mathcal{M}\downarrow$  &   0.051 
			&0.043 
			&0.046 
			&0.041 
			&0.040 
			&0.039 
			&0.041 
			&0.039 
			&0.041 
			&0.041 
			&0.040 
			&0.039 
			&0.037 
			&0.038 
			&0.037 
			&0.037 
			&0.045 
			& 0.037
			&0.037 
			& \color{myblue} \textbf{0.033} 
			& \color{mygreen} \textbf{0.032} 
			& \color{reda} \textbf{0.031} 
			& \color{myblue} \textbf{0.033} 
   
			\\
   				&$AUC\uparrow$ 
&.9798
&.9846
&.9785
&.9841
&.9846
&.9762
&.9804
&\color{myblue} \textbf{.9870}
&.9854
&.9742
&.9849
&.9567
&.9740
&.9849
&.9812
&.9806
&.9355
&.9832
&.9775
&\color{mygreen} \textbf{.9873}
&\color{reda} \textbf{.9884}
&.9818
&.9820
			\\
			\hline
			\multirow{5}{*}{\emph{\rotatebox{90}{NLPR}}}      
			&$F_{\beta}^{max}\uparrow$    &   0.910 
			&0.913 
			&0.921 
			&0.927 
			&0.925 
			&0.916 
			&0.925 
			&0.917 
			&0.927 
			&0.925 
			&0.919 
			&0.916 
			&0.917 
			&0.917 
			&0.927 
			&0.926 
			&0.898 
			& 0.929
			&0.898 
			& \color{myblue} \textbf{0.931} 
			&\color{mygreen} \textbf{0.935} 
			& \color{myblue} \textbf{0.931} 
			&\color{reda} \textbf{0.937} 
			\\
			&$F_{\beta}^{w}\uparrow$    &   
			0.852 
			&0.856 
			&0.871 
			&0.879 
			&0.882 
			&0.878 
			&0.881 
			&0.869 
			&0.882 
			&0.882 
			&0.877 
			&0.881 
			&0.886 
			&0.881 
			&0.889 
			&\color{mygreen} \textbf{0.896} 
			&0.857 
			& \color{myblue} \textbf{0.895}
			&0.842 
			&0.885 
			& {0.894} 
			& {0.893} 
			& \color{reda} \textbf{0.900} 
			\\
			& $S_m\uparrow  $         &  
			0.915 
			&0.917 
			&0.923 
			&0.930 
			&0.925 
			&0.920 
			&0.930 
			&0.916 
			&0.923 
			&0.930 
			&0.925 
			&0.918 
			&0.921 
			&0.921 
			&0.929 
			&0.927 
			&0.898 
			&0.929
			&0.908 
			&0.927 
			& \color{mygreen} \textbf{0.937} 
			& \color{myblue} \textbf{0.933} 
			& \color{reda} \textbf{0.938}
			\\
			& $E_m\uparrow$  &  
			0.942 
			&0.941 
			&0.948 
			&0.954 
			&0.955 
			&0.955 
			&0.955 
			&0.948 
			&0.957 
			&0.954 
			&0.954 
			&0.952 
			&0.956 
			&0.952 
			& \color{myblue} \textbf{0.959} 
			& \color{myblue} \textbf{0.959} 
			&0.945 
			&\color{mygreen} \textbf{0.961}
			&0.934 
			&0.952 
			& {0.958} 
			&{0.958} 
			& \color{reda} \textbf{0.963} 
			\\
			&$\mathcal{M}\downarrow$    & 
			0.030 
			&0.029 
			&0.026 
			&0.023 
			&0.022 
			&0.025 
			&0.024 
			&0.027 
			&0.023 
			&0.024 
			&0.024 
			&0.024 
			&0.023 
			&0.025 
			& \color{myblue} \textbf{0.022} 
			& \color{mygreen} \textbf{0.021} 
			&0.029 
			& \color{mygreen} \textbf{0.021} 
			&0.031 
			&0.024 
			& \color{mygreen} \textbf{0.021} 
			&\color{myblue} \textbf{0.022} 
			& \color{reda} \textbf{0.020} 
   			\\
   				&$AUC\uparrow$ 
&.9829
&.9866
&.9838
&.9882
&.\color{myblue} \textbf{9889}
&.9832
&.9878
&.9861
&.9888
&.9854
&\color{mygreen} \textbf{.9894}
&.9712
&.9770
&.9842
&.9846
&.9833
&.9447
&.9847
&.9826
&.9878
&\color{reda} \textbf{.9915}
&.9847
&.9867

			\\
			\hline
			\multirow{5}{*}{\emph{\rotatebox{90}{NJUD}}}      
			&$F_{\beta}^{max}\uparrow$   &   
			0.899 
			&0.913 
			&0.926 
			&0.931 
			&0.912 
			&0.908 
			&0.918 
			&0.924 
			&0.922 
			&0.919 
			&0.921 
			&0.917 
			&0.917 
			&0.920 
			&0.923 
			&0.935 
			&0.890 
			&0.911
			&0.902 
			&\color{myblue} \textbf{0.939} 
			&0.938 
			& \color{mygreen} \textbf{0.940} 
			& \color{reda} \textbf{0.945} 
			\\
			&$F_{\beta}^{w}\uparrow$     & 
			0.842 
			&0.857 
			&0.878 
			&0.884 
			&0.869 
			&0.868 
			&0.872 
			&0.881 
			&0.877 
			&0.878 
			&0.879 
			&0.883 
			&0.878 
			&0.879 
			&0.886 
			& \color{mygreen} \textbf{0.906} 
			&0.843 
			&0.872
			&0.850 
			&0.900 
			&0.900 
			& \color{myblue} \textbf{0.905} 
			& \color{reda} \textbf{0.909} 
			\\
			& $S_m\uparrow$        &   
			0.894 
			&0.903 
			&0.916 
			&0.921 
			&0.902 
			&0.897 
			&0.909 
			&0.911 
			&0.908 
			&0.913 
			&0.912 
			&0.904 
			&0.903 
			&0.909 
			&0.916 
			&0.924 
			&0.871 
			&0.902
			&0.895 
			& \color{mygreen} \textbf{0.928} 
			& \color{mygreen} \textbf{0.928} 
			& \color{myblue} \textbf{0.927} 
			& \color{reda} \textbf{0.930} 
			
			\\
			& $E_m\uparrow$     &   
			0.917 
			&0.923 
			&0.937 
			&0.942 
			&0.935 
			&0.934 
			&0.935 
			&0.934 
			&0.932 
			&0.940 
			&0.937 
			&0.937 
			&0.941 
			&0.931 
			&0.942 
			& \color{mygreen} \textbf{0.953} 
			&0.916 
			&0.936
			&0.924 
			&0.944 
			&0.944 
			& \color{myblue} \textbf{0.950} 
			& \color{reda} \textbf{0.954} 
			\\
			&$\mathcal{M}\downarrow$  &  
			0.053 
			&0.046 
			&0.039 
			&0.035 
			&0.041 
			&0.043 
			&0.042 
			&0.037 
			&0.038 
			&0.038 
			&0.039 
			&0.039 
			&0.038 
			&0.038 
			&0.037 
			& \color{reda} \textbf{0.029} 
			&0.047 
			&0.042 
			&0.046 
			&0.033 
			&0.033 
			& \color{myblue} \textbf{0.031} 
			& \color{mygreen} \textbf{0.030} 
      			\\
   				&$AUC\uparrow$ 
&.9745
&.9821
&.9828
&.\color{myblue} \textbf{9849}
&.9812
&.9700
&.9765
&.9843
&.9835
&.9766
&.9845
&.9619
&.9660
&.9810
&.9791
&.9814
&.9296
&.9739
&.9755
&\color{reda} \textbf{.9879}
&\color{mygreen} \textbf{.9872}
&.9825
&.9832

			\\
			\hline
			\multirow{5}{*}{\emph{\rotatebox{90}{SIP}}}      
			&$F_{\beta}^{max}\uparrow$   &   0.891 
			&0.890 
			&0.892 
			&0.902 
			&0.904 
			&0.896 
			&0.893 
			&0.904 
			&0.910 
			&0.888 
			&0.904 
			&0.891 
			&0.900 
			&0.916 
			&0.906 
			&0.916 
			&0.855 
			&0.900
			&0.883 
			& \color{mygreen} \textbf{0.935} 
			&0.929 
			& \color{myblue} \textbf{0.931} 
			& \color{reda} \textbf{0.937} 
			\\
			&$F_{\beta}^{w}\uparrow$   &   0.819 
			&0.811 
			&0.820 
			&0.830 
			&0.844 
			&0.836 
			&0.822 
			&0.835 
			&0.848 
			&0.812 
			&0.842 
			&0.829 
			&0.841 
			&0.854 
			&0.845 
			&0.868 
			&0.780 
			&0.836
			&0.803 
			& \color{myblue} \textbf{0.878} 
			&0.875 
			& \color{mygreen} \textbf{0.881} 
			& \color{reda} \textbf{0.893} 
			\\
			& $S_m\uparrow$        &   0.872 
			&0.867 
			&0.874 
			&0.879 
			&0.880 
			&0.875 
			&0.876 
			&0.878 
			&0.886 
			&0.862 
			&0.885 
			&0.862 
			&0.873 
			&0.886 
			&0.885 
			&0.894 
			&0.828 
			&0.877 
			&0.858 
			& \color{myblue} \textbf{0.909} 
			& \color{mygreen} \textbf{0.911} 
			& \color{myblue} \textbf{0.909} 
			& \color{reda} \textbf{0.917} 
			\\
			& $E_m\uparrow$     &  
			0.913 
			&0.909 
			&0.912 
			&0.917 
			&0.923 
			&0.918 
			&0.912 
			&0.921 
			&0.925 
			&0.905 
			&0.925 
			&0.911 
			&0.921 
			&0.925 
			&0.924 
			&0.931 
			&0.890 
			&0.923
			&0.909 
			& \color{myblue} \textbf{0.942} 
			&0.939 
			& \color{mygreen} \textbf{0.943} 
			& \color{reda} \textbf{0.950} 
			\\
			&$\mathcal{M}\downarrow$  &   0.057 
			&0.062 
			&0.056 
			&0.055 
			&0.049 
			&0.051 
			&0.055 
			&0.050 
			&0.047 
			&0.060 
			&0.049 
			&0.057 
			&0.052 
			&0.048 
			&0.048 
			&0.043 
			&0.070 
			&0.051
			&0.063 
			& \color{myblue} \textbf{0.039} 
			& \color{mygreen} \textbf{0.038} 
			& \color{mygreen} \textbf{0.038} 
			& \color{reda} \textbf{0.034} 
         			\\
   				&$AUC\uparrow$ 
&.9585
&.9524
&.9539
&.9555
&.9575
&.9528
&.9610
&.9660
&.9676
&.9361
&.9667
&.9328
&.9391
&.9607
&.9550
&.9609
&.8974
&.9625
&.9485
&\color{reda} \textbf{.9751}
&\color{myblue} \textbf{.9749}
&.9682
&\color{mygreen} \textbf{.9750}

			\\
			\hline
			\multirow{5}{*}{\emph{\rotatebox{90}{LFSD}}}      
			&$F_{\beta}^{max}\uparrow$   
			& 0.862 
			& \color{mygreen} \textbf{0.900} 
			&0.862 
			&0.879 
			&0.887 
			&0.878 
			&0.874 
			&0.860 
			&0.883 
			&0.879 
			&0.888 
			& \color{reda} \textbf{0.903} 
			&0.878 
			&0.877 
			&0.879 
			&0.881 
			&0.858
			&0.845 
			&0.877 
			&0.892 
			&0.895 
			& \color{myblue} \textbf{0.897} 
			&0.884 
			
			
			\\
			&$F_{\beta}^{w}\uparrow$    
			& 0.772 
			&0.834 
			&0.789 
			&0.814 
			&0.822 
			&0.832 
			&0.800 
			&0.792 
			&0.806 
			&0.821 
			&0.827 
			& \color{reda} \textbf{0.859} 
			&0.824 
			&0.811 
			&0.816 
			&0.823 
			&0.800 
			&0.775
			&0.815 
			&0.821 
			& \color{myblue} \textbf{0.839 }
			& \color{mygreen} \textbf{0.843} 
			&0.827 
			
			\\
			& $S_m\uparrow$  
			& 0.837 
			&0.876 
			&0.845 
			&0.864 
			&0.862 
			&0.864 
			&0.853 
			&0.847 
			&0.854 
			&0.859 
			&0.870 
			& \color{reda} \textbf{0.883} 
			&0.856 
			&0.854 
			&0.858 
			&0.854 
			&0.833 
			&0.827
			&0.862 
			&0.868 
			& \color{mygreen} \textbf{0.881} 
			& \color{myblue} \textbf{0.877} 
			&0.871 
			
			
			\\
			& $E_m\uparrow$    &
			0.876 
			& \color{myblue} \textbf{0.908} 
			&0.883 
			&0.901 
			&0.902 
			&0.906 
			&0.894 
			&0.883 
			&0.891 
			&0.899 
			&0.906 
			& \color{reda} \textbf{0.923} 
			&0.903 
			&0.892 
			&0.898 
			&0.897 
			&0.875 
			&0.869
			&0.901 
			&0.900 
			& \color{mygreen} \textbf{0.909} 
			& \color{mygreen} \textbf{0.909} 
			&0.897 
			
			\\
			&$\mathcal{M}\downarrow$  &   0.094 
			&0.066 
			&0.080 
			&0.072 
			&0.070 
			&0.066 
			&0.074 
			&0.085 
			&0.077 
			&0.073 
			&0.068 
			& \color{reda} \textbf{0.055} 
			&0.071 
			&0.079 
			&0.073 
			&0.071 
			&0.077 
			&0.099
			&0.071 
			&0.072 
			& \color{myblue} \textbf{0.064} 
			& \color{mygreen} \textbf{0.063} 
			&0.066 
         			\\
   				&$AUC\uparrow$ 
&.9614
&.9734
&.9468
&.9697
&.9668
&.9570
&.9624
&.9640
&.9727
&.9532
&\color{myblue} \textbf{.9741}
&.9611
&.9460
&.9662
&.9606
&.9576
&.9087
&.9475
&.9594
&\color{mygreen} \textbf{.9746}
&\color{reda} \textbf{.9754}
&.9681
&.9625
	
			\\

			\bottomrule[2pt]
		\end{tabular}

==> table/param_flops_response.tex <==

 \begin{tabular}{r||cccccccccccccc}
\toprule[1.5pt]
% \rowcolor{mygray}
		Model Nmae  &{CDNet$_{21}$} &{DFMNet$_{21}$} &{DSA2F$_{21}$} &{DCF$_{21}$}&{HAINet$_{21}$} &   {RD3D$_{21}$} &   {SPNet$_{21}$} & {A2DELE$_{20}$}&{DASNet$_{20}$}&{CoNet$_{20}$} & {MMFT} &{MMFT} & {MMFT} & {MMFT} \\
		Backbone  &VGG-16 &ResNet-34& VGG-19& ResNet-50& VGG-16& ResNet-50& Res2Net-50&  VGG-16& ResNet-50&ResNet-101& VGG-16& ResNet-50& Res2Net-50& ResNet-101 \\
	\midrule[1pt]
		Parameters (MB)$\downarrow$    & \color{myblue}\textbf{32.93} &\color{mygreen}\textbf{23.44} & 36.48 & {47.85} & 59.82 &{46.90}&\textbf{150.31}&\color{reda}\textbf{14.90}&{36.68}&43.66& {41.38}&53.12&{75.96}&72.13
		\\
		FLOPs (G)$\downarrow$     &{72.10} & 26.32 &{172.23} &\color{reda}\textbf{17.74} & \textbf{181.41} & 50.72 &{67.92}&39.07&{28.56}&{27.37}&72.82&\color{mygreen}\textbf{20.32}&25.89&\color{myblue}\textbf{25.50}
		\\
 \bottomrule[1.5pt]
	\end{tabular}

